"Because Some Sighted People, They Don't Know What the Heck You're Talking About:" A Study of Blind TikTokers' Infrastructuring Work to Build Independence

There has been extensive research on the experiences of individuals with visual impairments on text- and image-based social media platforms, such as Facebook and Twitter. However, little is known about the experiences of visually impaired users on short-video platforms like TikTok. To bridge this gap, we conducted an interview study with 30 BlindTokers (the nickname of blind TikTokers). Our study aimed to explore the various activities of BlindTokers on TikTok, including everyday entertainment, professional development, and community engagement. The widespread usage of TikTok among participants demonstrated that they considered TikTok and its associated experiences as the infrastructure for their activities. Additionally, participants reported experiencing breakdowns in this infrastructure due to accessibility issues. They had to carry out infrastructuring work to resolve the breakdowns. Blind users' various practices on TikTok also foregrounded their perceptions of independence. We then discussed blind users' nuanced understanding of the TikTok-mediated independence; we also critically examined BlindTokers' infrastructuring work for such independence.

==> Sections/2_Background.tex <==
\section{Background: A Brief Introduction of TikTok [Delete]}
TikTok is a gigantic platform that offers a wide variety of services, and it is impossible to fully demonstrate all the services it provides in this section. Therefore, based on the stories reported by the participants and the authors' experiences, we demonstrate functions and designs that are relevant to the experiences of blind users.

The primary interface of TikTok includes a video that almost occupies the entire screen, buttons, such as the video creator's profile picture, "like" "comment" and "share," on the left side, and the titles, descriptions, and hashtags of the video at the bottom, and "following," "for you" at the top (Figure \ref{fig:1}, a). To view one's homepage, users can click on their profile pictures or names. The homepage presents the username, the bio, and the videos published (Figure \ref{fig:1}, b). Viewers can share the page through links, SMS, or messages. Creators can select and pin certain videos at the top of the page. At the bottom of the primary interface, users can hit the "+" button to start creating videos (Figure \ref{fig:1}, a). On the video creation page, users can use the phone camera to take videos and add visual and/or audio effects (Figure \ref{fig:1}, c). 

In addition to adding effects, TikTok also has functions that make creating videos more playful. For instance, users can create videos of their faces and then let the algorithm match the faces with characters from cartoons, movies, etc. (Figure \ref{fig:1}, d). To enhance the viewer experience, creators can also add captions to their videos (Figure \ref{fig:1}, f). TikTok also allows users to interact with others through various functions such as live-streaming, stitch, and duets. The live-steaming interface is similar to the interface for displaying videos; the main difference is that it displays the commenting and gifting behaviors of viewers in real-time, so the lower part of the interface automatically scrolls to present the most recent comments or gifts (Figure \ref{fig:1}, e). Duet is a type of activity that requires users to create videos collaboratively. One user creates a video in advance, and another user "duets" it by putting the video on the right side of the screen and creating another according to the previous one. Usually, duets are manifested as co-performance like singing or dancing together. For collaborative singing, sometimes singers who create videos for later people to duet use different colors to mark the lyrics so that later creators know which part they need to sing (Figure \ref{fig:1}, f).

As we can learn from the brief introduction of TikTok, it is a highly visual-oriented platform. Many user experiences involve the recognition of text, color, or images. In addition, to make the image or video content as large as possible on the screen, TikTok chose small, low-contrast, and relatively transparent text fonts, icons, and buttons so that they will not overlap with the video/image content. In fact, TikTok's design significantly affected the experiences of blind users, as participants complained. We will present a detailed description of blind users' experiences on TikTok in the Findings section. 

%How blind people use most social media
%[reply with video; put the comment on the video]


%\subsection{Video Browsing, Creating}
%\subsection{TikTok Gaming: Stitching, Duet, Other Challenges}
%\subsection{Comments, Share, Message} Font is small

%Update a lot


\begin{figure}[htp]
    \centering
    \includegraphics[width=15cm]{Figures/Background/TikTok-Interface.png}
    \caption{TikTok's Primary Interface (a), User Homepage (b), Video Filter (c), Character Matching (d), Live-streaming (e), and Duet (f).}
    \label{fig:1}
\end{figure}


